Non-Contrastive Learning-based Behavioural Biometrics for Smart IoT Devices

Behaviour biometrics are being explored as a viable alternative to overcome the limitations of traditional authentication methods such as passwords and static biometrics. Also, they are being considered as a viable authentication method for IoT devices such as smart headsets with AR/VR capabilities, wearables, and erables, that do not have a large form factor or the ability to seamlessly interact with the user. Recent behavioural biometric solutions use deep learning models that require large amounts of annotated training data. Collecting such volumes of behaviour biometrics data raises privacy and usability concerns. To this end, we propose using SimSiam-based non-contrastive self-supervised learning to improve the label efficiency of behavioural biometric systems. The key idea is to use large volumes of unlabelled (and anonymised) data to build good feature extractors that can be subsequently used in supervised settings. Using two EEG datasets, we show that at lower amounts of labelled data, non-contrastive learning performs 4%-11% more than conventional methods such as supervised learning and data augmentation. We also show that, in general, self-supervised learning methods perform better than other baselines. Finally, through careful experimentation, we show various modifications that can be incorporated into the non-contrastive learning process to archive high performance.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> sections/Experiments.tex <==
\section{Experiments}
\label{Sec:Experiments}






\subsection{Dataset Splits}

% From here onward, for all our experiments, we will be dividing the dataset into two parts. This division is done to emulate real-world scenarios. {\bf Dataset 1} contains data from 6 users, approximately 1/3 of the users from the total dataset. {\bf Dataset 2} contains data from 14 users, approximately 2/3 of the users from the total dataset.\\ \vspace{-3mm}

% {\bf Dataset 1} is used to replicate a dataset seen in the product development stage or an initial model building stage. It has a low number of users with many unlabeled samples and few labeled samples. When we are initially building a model, we have the freedom to gather a lot of data in an experimental environment. However, we will not have the luxury of labeling all those samples due to privacy and security constraints. In most cases, we will only be able to record data from fewer users than the number of users the model will meet once the model is deployed. So, we will be left with a limited number of users, each providing lot of unlabeled data and a few labeled data. To replicate this scenario, we pick six users (nearly 1/3 of the total users) with the highest number of recorded sessions in the dataset.\\ \vspace{-3mm} 

% {\bf Dataset 2} is used to replicate a dataset that can be seen in a product use case. This dataset has a higher number of users compared to Dataset 1. In our case, more than twice the number of users in Dataset 1. Each user will only have a limited number of samples. When we register a user to a device using biometric data, we cannot ask the user to provide us with many samples. It is against user convenience, which is one of the most significant factors that decide the quality of a mobile or IoT device. It also raises questions about privacy and security. So practically, if we are adding users to a device, we will be left with only a limited number of labelled samples from each user and some unlabelled data. If we take an IoT device installed in a facility with a large number of workers, we will be left with a dataset with many users, each having only a limited number of labelled samples. To replicate this scenario, we pick 14 users (nearly 2/3 of the total users) with the lowest number of recorded sessions.

% \noindent{\bf 2. Scenarios}\\ \vspace{-3mm} 

% We define three scenarios to evaluate the performance of self-supervised learning in behavioral biometrics based authentication tasks.


% \begin{enumerate}[label=\roman*.]
%     \item {\bf Scenario 1} replicates a situation where there is a dataset containing many unlabelled samples from some user. Only a few labeled samples are available from those users. One should be able to build an accurate user authentication system for those users by utilizing both unlabelled and labeled data.\\
%     {\it -In other words, the model will only have access to a database similar to {\bf Dataset 2}.}\\ \vspace{-3mm}
    
%     \item {\bf Scenario 2} emulates a user addition scenario to an already existing authentication system. Only a few labeled data will be available from the new users, and no unlabelled data. An authentication system should be able to add new users with a minimum labeled data requirement.\\
%     {\it -We will have access to a database similar to {\bf Dataset 1} to build an initial model. Afterward, we will be given a database similar to {\bf Dataset 2} with news users that need to be added to the authentication model.}\\
%     \vspace{-3mm}
    
%     \item {\bf Scenario 3} contains lots of unlabelled data from few users and few labeled samples from another set of users. The latter will have more users than the former. An authentication system should be able to authenticate the second set of users with a minimum data requirement. These systems have the freedom to utilize the unlabelled data from the first set of users as they desire.\\
%     {\it -We will have access to a database similar to {\bf Dataset 1} which does not contain any labelled data. End goal is to build an authentication model for the users in a database similar to {\bf Dataset 2}. But we have the freedom to utilize the unlabelled data from {\bf Dataset 1}.}\\
%     \vspace{-3mm}
% \end{enumerate}

% \noindent{\bf 3. Experimental Setups of the Three Scenarios}\\ \vspace{-3mm}

% Here we describe how we experimentally execute the three scenarios mentioned above and compare the performances of self-supervised models in each scenario. Each end-classifier is trained with different {\bf number of samples per user} values ranging from 1 to 60.\\ \vspace{-3mm}.

% \noindent{\bf Scenario 1}\\ \vspace{-3mm}

% In scenario 1 we compare four methods. Supervised learning and Supervised learning with data augmentations are used as baseline models. These baseline models are unable to utilize the unlabelled data available. In contrast to them the two self-supervised models are able to utilize the unlabelled data.

% \begin{enumerate}[label=\roman*.]
%   \item {\bf Supervised Learning Baseline}: An end-to-end supervised DNN is trained using the {\bf Dataset 2} as a baseline. This supervised model is a concatenation of the feature extractor and the classifier networks.
%   \item {\bf Data Augmentation Baseline}: An end to end supervised DNN is trained using the {\bf Dataset 2} as same as the Supervised Learning Baseline. As an improvement, we apply data augmentations to the input data to overcome the low data availability.
%   \item {\bf Self Supervised Multi Task Learning( {\it SSMT} )}: A self-supervised multi-headed model is trained using the whole {\bf Dataset 2} but without using any labels. Then the learned feature extractor is extracted from the {\it SSMT}, and it is used to train the classifier on top of it. Few labeled samples from the {\bf Dataset 2} is used to train the classifier.
%   \item {\bf Simple Siamese Network( {\it SimSiam} )}: The feature extractor is trained using the SimSiam network. The rest is trained in the same way as the {\it SSMT} model.
% \end{enumerate}

% We want to mention that we are not using users from {\bf Dataset 1} in this scenario. We are doing this because we want to compare the performances of self-supervised models between Scenario 1 and Scenario 3. This will be discussed in the section {\bf User Independent representation learning using self-supervised methods.}\\ \vspace{-3mm}

% \noindent{\bf Scenario 2}\\ \vspace{-3mm}

% In scenario 2 we compare the performance of four methods. Transfer learning and transfer learning with augmentation are unable to utilize the unlabelled data. In contrast to that, the two self-supervised methods are able to utilize the unlabelled data.\\
% In each method, we train an initial classifier for the users in {\bf Dataset 1}.
% Furthermore, this initial training process is done by using a minimum amount of data. We do this by training each initial classifier with different {\bf number of samples per user} values starting from 1 and increasing. We do this until the classifier is able to achieve a threshold accuracy. In our experiment, we use {\bf 0.95} as the threshold.\\
% Then we add new users to each classifier. We do this by fine-tuning the initial model for users from both {\bf Dataset 1} and {\bf Dataset 2}. Here we have to mention that we replace the classification network that is already trained with {\bf Dataset 1} with a randomly initialized new network. We observed a considerable accuracy drop while using a pre-trained classification network.

% \begin{enumerate}[label=\roman*.]
%   \item {\bf Transfer Learning}: Initially, an end-to-end supervised DNN is trained using the {\bf Dataset 1} for the users in that dataset. This DNN has the same architecture as the supervised DNN used in scenario 1. After the initial training, we add new users from the {\bf Dataset 2} by taking the learned feature extractor from the initial model and retraining(fine-tuning) the model with the newly attached classifier.
%   \item {\bf Transfer Learning with Data Augmentations}: The initial model is trained in the same way as mentioned in the Transfer Learning scenario, but with data augmentations applied to inputs. New user addition is also done in the same way but with data augmentations. Data augmentations are used to achieve the low data requirement for the model.
%   \item {\bf Self Supervised Multi Task Learning( {\it SSMT} )}: A self-supervised multi-headed model is trained using the whole {\bf Dataset 1} but without using any labels. Then the learned feature extractor is extracted from the {\it SSMT}, and it is used to train the classifier(using {\bf Dataset 1}) on top of it. After training the initial classifier, we add new users from {\bf Dataset 2} by again fine-tuning the already fine-tuned feature extractor with a newly attached classifier.
%   \item {\bf Simple Siamese Network( {\it SimSiam} )}: The feature extractor is trained using the SimSiam network. The rest is trained in the same way as the {\it SSMT} model.
% \end{enumerate}

% \noindent{\bf Scenario 3}\\ \vspace{-3mm}

% In this scenario we compare five methods. Supervised learning and supervised learning with augmentations are used as baselines and both of them are unable to utilize data from {\bf Dataset 1}. Two self-supervised methods are able to utilize unlabelled data from {\bf Dataset 1}. Although the transfer learning method violates the rules we defined for scenario 3 by using user labels of {\bf Dataset 1}, We still use the transfer learning to compare the representation learned by the self-supervised methods. Through that comparison we show how good is a representation learned using self-supervision tasks compared to a representation learned using end task of the classifier.

% \begin{enumerate}[label=\roman*.]
%   \item {\bf Supervised Learning Baseline}: This is trained in the same way as mentioned in Scenario 1.
%   \item {\bf Data Augmentation Baseline}: This is trained in the same way as mentioned in Scenario 1.
%   \item {\bf Transfer Learning}: An end-to-end supervised DNN is trained using the {\bf Dataset 1} for the users in that dataset. This DNN has the same architecture as the supervised DNN used in scenario 1. Then the learned feature extractor is used to train the classifier on top of it. Few labeled samples from the {\bf Dataset 2} are used to train the classifier.
%   \item {\bf Self Supervised Multi-Task Learning( {\it SSMT} )}: Feature extractor is trained using the SSMT model. The rest is trained in the same way as the Transfer Learning model.
%   \item {\bf Simple Siamese Network( {\it SimSiam} )}: Feature extractor is trained using the SimSiam Network. The rest is trained in the same way as the Transfer Learning model.
% \end{enumerate}




==> sections/Related.tex <==
\section{Related Work}
\label{Sec:Related}

\subsection{Behavioural Biometrics}

There is a vast body of work proposing various behavioural biometric modalities. Early work involved active human input ~\cite{banerjee2012biometric,10.1145/3372224.3380901,meng2014design} while later modalities depended on human physiology ~\cite{chauhan2017breathprint,chauhan2018breathing,sooriyaarachchi2020musicid,zhang2018mindid,zhao2020trueheart,vhaduri2017wearable}. In general, two main types of authentication mechanisms have been tested with these modalities; \textit{user identification} and \textit{user verification}~\cite{abuhamad2020sensor}.  Both cases involve building machine learning classifiers or  signature similarity-based approaches~\cite{abuhamad2020sensor} although more recent work uses deep learning methods~\cite{sundararajan2018deep} given their broader success in other domains. 

Other works in behavioural biometrics aimed to increase the usability and the training efficiency. Chauhan et al.~\cite{chauhan2020contauth} implemented deep learning with data incremental learning and class incremental learning - removing the need to retrain models for new users or changes in existing user behaviour. Others worked towards improving the label efficiency using few-shot learning ~\cite{solano2020few} and transfer-learning ~\cite{zhang2021human}. Similar efforts were made in human activity recognition~\cite{sheng2019siamese, saeed2019multi}.


%using keyboard typing patterns~\cite{banerjee2012biometric}. Later with the popularity of touch screens in smart devices, multiple work showed that user touch patterns measured by features in the likes of touch pressure~\cite{10.1145/3372224.3380901,meng2014design} can be used to uniquely identify a user. Several other work explored the modalities driven by human physiology such as breathing acoustics~\cite{chauhan2017breathprint,chauhan2018breathing}, EEG patterns~\cite{sooriyaarachchi2020musicid,zhang2018mindid}, and heart rate~\cite{zhao2020trueheart,vhaduri2017wearable} as means of user authentication. Another set of work demonstrated that human walking patterns and various gestures as measured by a smartphone's accelerometer and gyroscope and also be used to identify a user~\cite{cola2016gait,yang2015motionauth,wu2013dynamic}.


%In general, two main types of authentication mechanisms have been tested with these modalities; \textit{user identification} and \textit{user verification}~\cite{abuhamad2020sensor}. In user identification, a user is identified from a closed-set of users solely based on a behavioural modality. In user verification, it is assumed that the users attempt to verify themselves by providing some identification number in addition to behavioural biometric data samples. In both cases the approach is to build machine learning classifiers (multi-class for user identification and binary for user verification), or use signature similarity-based approaches~\cite{abuhamad2020sensor}.  More recent work in behavioural biometrics used deep learning methods~\cite{sundararajan2018deep} due to their broader success in other domains.

%\textcolor{blue}{P3 - } \textcolor{red}{discuss the improvements such as continuous authentication, learning with less data, .... any other work that goes beyond than proposing a new modality.}

%Other works in behavioural biometrics proposed methods to increase the usability and the training efficiency. Chauhan et al.~\cite{chauhan2020contauth} combined deep learning models with online learning to implement data incremental learning and class incremental learning - removing the need to retrain models for new users or changes in existing user behaviour. Others work towards improving the label efficiency (i.e., reducing the amount of labelled training data). Examples involve using few-shot learning ~\cite{solano2020few} and transfer-learning ~\cite{zhang2021human}. Although not in the user authentication, similar efforts were made in human activity recognition~\cite{sheng2019siamese, saeed2019multi}.

\textit{In contrast, we propose non-contrastive learning to improve the label efficiency when training behavioural biometric model. Non-contrastive learning enables leveraging large volumes of unlabelled data to build label-efficient classifiers. To the best of our knowledge, our work is the first to use non-contrastive learning for behavioural biometrics.}

\subsection{Self-supervised Learning (SSL)}

Self-supervised learning (SSL) is currently a highly active area of machine learning. It refers to a broader a family of methods in which a model learns representations from unlabelled data using \textit{pretext tasks}. The objective of pretext task based learning is that, it can subsequently act as a feature extractor for supervised learning tasks, and the labelled data requirement can be reduced. For example, in computer vision, a pretext task can be image augmentation (e.g., rotation, noise addition, clipping, and resizing) and during pretext task learning, a model is trained to predict whether a given image is augmented or not. Next, the pretext model is extended to a supervised setting with labelled data. Jing et al.~\cite{jing2020self} provides a survey of SSL methods. 

Though there has been early work related to SSL, the most closest idea to modern SSL is the work by Bromley et al.~\cite{bromley1993signature}, where the authors proposed the "Siamese" neural network architecture for signature verification. Because of excessive resource requirements, SSL didn't receive much attention until they have been effectively used in natural language processing in the last decade~\cite{he2020momentum, chen2020simple,mao2020survey, li2022tribyol}. In 2013, Mikolov et al.~\cite{mikolov2013distributed} used self-supervised learning to represent words in a vector space, famously known as \textit{word2vec}. This idea of masked language models, paved the way to a significant amount of subsequent language models such as BERT~\cite{devlin2018bert}, RoBERTa~\cite{liu2019roberta} and XLM-R~\cite{conneau2019unsupervised}. In masked language models, which is a generative self-supervised learning method, a segment of a sentence or a paragraph is masked, and the model is trained to predict the contents of the masked segment.

Nonetheless, \textit{generative methods}~\cite{hinton2006fast, kingma2013auto, goodfellow2014generative} (i.e., using pretext tasks generate a feature, the input, or parts of the input) were not successful in other domains such as computer vision because of their high computational complexity~\cite{chen2020simple}. Neither were \textit{discriminative approaches}~\cite{doersch2015unsupervised, zhang2016colorful, noroozi2016unsupervised, gidaris2018unsupervised} (i.e., using pretext tasks  to classify whether a known transformation is applied to inputs), because they relies on heuristics to design pretext tasks limiting the generality of the learnt representation~\cite{chen2020simple}. In contrast, Siamese networks-based \textit{comparative methods} (i.e., pretext tasks try to increase the similarity for given two inputs of same type) have shown promising results in computer vision~\cite{chen2020simple, grill2020bootstrap, caron2020unsupervised, chen2021exploring}.


% P3 - In Siamese networks, we have two identical networks. Sometimes one network can be a moving average of the other network. We try to reduce the energy between embeddings of two views of the same sample. The two embeddings are the outputs of the identical networks when two views of the same sample are given as inputs to each. Energy is the output of a function that indicates the two embeddings' compatibility(or similarity). Low energy means high compatibility and vice versa. The two views can be either two augmented versions(spatial) of the same sample or two instances of the same sample with a time delay(temporal). In order to increase the similarity of the two views, the networks should learn a spatial or temporal transformation invariant embedding. However, these kinds of Siamese networks suffer from a phenomenon called collapsing networks, where the network archives a trivial solution. If the network outputs the same embedding for everything regardless of the input, energy between any two pairs will be reduced to the minimum. To avoid this trivial solution, contrastive models use negative pairs, and non-contrastive models use other sophisticated methods.

The basic form of Siamese networks, consists of two identical neural networks. The two networks take two views of the same input (i.e., a positive pair), and try to output embeddings that a have a low energy between them. Here, \textit{energy} refers to the output of a function that indicates the similarity or compatibility between the embeddings. The positive pair can be either two augmented versions of the same sample (spatial) or two instances of the same sample with a time delay (temporal). To increase the similarity of the two views, the networks must learn a spatial or temporal transformation invariant embeddings. Though there have been many successful applications of Siamese Networks~\cite{chen2020simple, grill2020bootstrap, caron2020unsupervised, chen2021exploring}, the phenomenon called \textit{collapsing networks}, where the network archives a trivial solution (i.e., both the networks produces exactly the same embedding irrespective of the input), limits their performance. 

To overcome the limitations of Siamese networks, \textit{contrastive learning} methods such as SimCLR~\cite{chen2020simple}, MoCo~\cite{he2020momentum}, NNCLR~\cite{dwibedi2021little}, PIRL~\cite{misra2020self}, and TS-TCC~\cite{eldele2021time} have been proposed. The key idea of contrastive learning is to use negatives to avoid collapsing by not only pulling positives towards each other, but also to pushing apart negatives in the embedding space (i.e., trying to decrease the energy between positive pairs while trying to increase energy between negative pairs at the same time). A negative pair consists of two different inputs, in contrast to a positive pair which is two views of the same input. However, contrastive learning approaches require large batch sizes (SimCLR~\cite{chen2020simple}, TS-TCC~\cite{eldele2021time}), support sets (NNCLR~\cite{dwibedi2021little}), or memory queues (PIRL~\cite{misra2020self}, MoCo v2~\cite{chen2020improved}, MoCo~\cite{he2020momentum}). As a result, \textit{non-contrastive learning} methods emerged as an viable alternative. In non-contrastive learning, instead of using negative pairs, other methods such as stop-gradient and a predictor (SimSiam~\cite{grill2020bootstrap}, BYOL ~\cite{chen2021exploring}), clustering (DeepCluster~\cite{caron2020unsupervised}, SwAV~\cite{caron2018deep}), and cross-correlation matrix between the outputs of
two identical networks as the objective function (Barlow Twins~\cite{zbontar2021barlow}) are used, which are efficient and simpler than contrastive approaches~\cite{tian2021understanding}.

% P5 - Aaqib et al. ~\cite{saeed2019multi} introduced self-supervised learning for time-series data by introducing augmentations that are compatible with time-series data. They use a Multi-Task Self-Supervised learning model to learn the embedding. They show their method's effectiveness using six human activity recognition data sets. Further details about this architecture will be discussed in the next section. Tang et al. ~\cite{tang2020exploring} have experimented with SimCLR architecture using HAR data. Qian et al. ~\cite{qian2022makes} explores BYOL, SimSiam, SimCLR, NNCLR( Dwibedi et al.~\cite{dwibedi2021little}), and TS-TCC(Eldele et al.~\cite{eldele2021time}) on HAR data. The effectiveness of self-supervised learning on time-series data has already been proven over and over in recent years.

\subsection{SSL in Sensing and Behavioural Biometrics}

While the majority of the work in SSL is happening in natural language processing, computer vision, and speech processing, recently multiple work explored its feasibility in sensing and mobile computing~\cite{tagliasacchi2019self}. For instance, Saeed et al.~\cite{saeed2019multi} introduced self-supervised learning for time-series sensor data by introducing augmentations that are compatible with time-series data. The authors use a multi-task SSL model to reduce the labeled training data requirement in Human Activity Recognition (HAR). They could achieve a kappa score between 0.7 - 0.8 only using 10 labeled samples per class, which was approximately 88.8\% of the highest score achived by conventional supervised learning. Tang et al. ~\cite{tang2020exploring} experimented with 81 combinations of signal transformations and showed that the SimCLR architecture can be used for HAR data. Similarly, Qian et al. ~\cite{qian2022makes} assessed the performance of several contrastive and non-contrastive SSL methods such as BYOL, SimSiam, SimCLR, NNCLR, and TS-TCC on HAR data. Cheng et al.~\cite{cheng2020subject} used a contrastive self-supervised method similar to MoCo~\cite{he2020momentum} to learn a subject invariant representation from ECG and EEG data. They use an adversarial training method remove subject specific characteristics from the representation. Several other works used self-supervised contrastive learning to obtain representations for time-series data such as ECG, EEG, and motion sensors~\cite{eldele2021time,mohsenvand2020contrastive,sarkar2020self,aggarwal2019adversarial}.

% They decompose contrastive models into several key components and conducted thorough investigation to understand how each component supports to achieve a better representation learning. \textcolor{red}{again good to say about any findings...?}\textcolor{violet}{ What they show is, these self-supervised methods can be used with HAR data and how each component affects learning a good representation.}

% Siamese networks have been explored in the domain of behavioral biometrics through rigorous experimentation~\cite{saeed2019multi, qian2022makes, tang2020exploring, eldele2021time, aggarwal2019adversarial, sarkar2020self, cheng2020subject, mohsenvand2020contrastive}. \textcolor{red}{Can you double check these work, some of them are not behavioural biometrics, e.g. activity recognition, and others have already been described e.g. 40. Whatever remaining add to the sentence in blue below.}

%Siamese networks have been explored in the domain of behavioral biometrics through rigorous experimentation~\cite{aggarwal2019adversarial}, 

% Subject-aware contrastive learning biosignals - ~\cite{cheng2020subject}
% Time-Series Representation Learning via Temporal and Contextual Contrasting~\cite{eldele2021time} Contrastive Representation Learning for Electroencephalogram Classification~\cite{mohsenvand2020contrastive}, Self-supervised ecg representation learning
% for emotion recognition~\cite{sarkar2020self}, Adversarial unsupervised representation learning for activity time-series~\cite{aggarwal2019adversarial}.

Several work explored the use of traditional Siamese networks to reduce the training data requirement of  behavioural-biometrics based user-authentication. For instance, Wright and Stewart~\cite{wright2019one} implemented a Siamese network architecture with one-shot-learning for lip-based biometric authentication and showed that it could outperform other known methods. In another work, Miller et al.~\cite{miller2021using} used a Siamese neural network, to allow users more seamless use of multiple virtual reality (VR) systems. The proposed approach enables cross-system user authentication when use-time data and user enrolment is provided over different VR systems, and therefore indirectly refers to the data availability issue. %\textcolor{red}{Subject-aware contrastive learning biosignals - ~\cite{cheng2020subject} - Can we write something about this work?} \textcolor{violet}{Since their work doesn't involve user authentication, I will add it to the previous paragraph}


%However both these papers focus on specific types of authentication whereas in this paper our methodology is tested using different types of biometric authentication datasets.}
% SimSiam~\cite{chen2021exploring}-based

\textit{In contrast to these works, to the best of our understanding, we are the first to propose  SimSiam~\cite{chen2021exploring}-based non-contrastive learning for behavioural biometrics to reduce the labeled data requirement. 
Compared to Siamese neural networks used in~\cite{wright2019one,miller2021using} and contrastive learning approaches for time series representation learning~\cite{cheng2020subject}, our method neither uses negatives nor requires complex training approaches such as momentum encoders to avoid collapsing. \textcolor{cyan}{The biggest disadvantage in using negatives in contrastive learning is samples from the same class getting pushed apart in the embedding space~\cite{khosla2020supervised}. As in contrastive learning a positive pair consist of two views of the same sample and all other samples in that mini-batch are considered as negatives, two samples from the same class can become a negative pair. It can harm the performance of the end task. Non-contrastive learning overcomes this problem by not using negatives.} We compare our approach with the traditional supervised learning, transfer learning, data augmentation, and state-of-the-art multi-task learning~\cite{saeed2019multi} and show that it can achieve competitive levels of label efficiency.} 
\textcolor{red}{We can come back to this again - There is a slight problem in this paragraph because later we don't talk about collapsing or any evidence of collapsing in other architectures. We also don't compare with SimCLR, right? Also, negatives can be generated without extra cost - Need to think of a more strong argument here.}\textcolor{violet}{Answered}

%ones to explore Multi-task self-supervised learning~\cite{saeed2019multi}(a discriminative SSL approach) and SimSiam~\cite{chen2021exploring} architecture(a non-contrastive SSL approach) to reduce the labeled data requirement of behavioral biometric based user authentication tasks.}

%\textcolor{red}{P2 - Next paragraph must be something along the below lines - The ideas behind SSL mainly stems from NLP where .... Talk about Word2Vec~\cite{mikolov2013distributed} (This is my thinking, but I can be wrong .. verify and write / On second thoughts Siamese networks are older than word2vec). Next we need some categorization of SSL methods, this can come from a survey paper; ...}

%\textcolor{red}{P3 - One of early ideas of SSL learning includes Siamese architectures~\cite{}. In Siamese networks, we have two identical networks. Sometimes one network can be a moving average of the other network. We try to reduce the energy between embeddings of two views of the same sample. We feed two views to the two identical networks. The outputs of the networks are the embeddings. Then we define a distance function(this can be considered the energy function), and we try to reduce the distance between the two views. Two views are usually two random augmentations of the same sample. In CV tasks, these augmentations are usually cropping out parts of the image, adding noise, scaling, rotation, flipping, color jitter, or a combination of a few augmentations. In order to increase the similarity of the two views, the networks should learn a transformation invariant embedding. In learning this transformation invariant embeddings, the network discovers important features or patterns that are useful in many downstream tasks. However, these kinds of Siamese networks suffer from a phenomenon called collapsing networks. If the network outputs the embedding for everything regardless of the input, energy between any two positive pairs will be reduced to zero.}

%\textcolor{red}{P4 - More recent ideas of SSL includes, multi-task learning~\cite{}, contrasting learning~\cite{}, and non-contrastive learning~\cite{}}.


%\textcolor{red}{P5 - Final paragraph has to be attempts of SSL in biometrics, behavioural biometrics, and sensor data. This can include the multi-task learning paper, Cecilia Mascolo's paper, The singapore paper and others ... (This can overlap with the section below, that we can sort out later) }

%In recent years self-Supervised gained a lot of popularity due to its' success in the domain of Natural Language processing. Some of the most famous language models that is trained using self-supervised learning are RoBERTa, XLM-R and BERT. In self-supervised learning we generate supervisory signal within our data by defining pre-text tasks. That is why the term "Unsupervised Learning" not in the use anymore.Because learning can never be unsupervised. In NLP models most commonly, the task is predicting a missing word in a middle of a sentence or predicting the next word of an unfinished sentence. There is a reason behind the success of NLP in self-supervised learning. There are only a finite number of words to select from to fill the blank. So these models can predict a probability distribution across all possible words and pick the word with the highest probability to complete the sentence. In other words, these pre-text tasks can be modeled as classification tasks. In contrast, computer vision tasks have an infinite number of possibilities. The task can be predicting a cropped-out part of an image, predicting a missing video frame, or predicting the next frame of a video. We have to do a pixel-level prediction of the missing part(part can be temporal or spatial).

%In the past few years, self-supervised learning started improving its' performance in computer vision with the revival of Siamese Networks in 2019. These networks can be classified into the so-called Energy-Based Models(EBM) category. Yann LeCun and Ishan Misra talk about EBMs in their blog about self-supervised learning in their Meta AI blogpost. The term EBM is adapted from classical physics. In a high-level view, these models try to reduce the energy between two positive samples and increase the energy between two negative samples. This energy is usually a loss function or a distance function.

%In Siamese networks, we have two identical networks. Sometimes one network can be a moving average of the other network. We try to reduce the energy between embeddings of two views of the same sample. We feed two views to the two identical networks. The outputs of the networks are the embeddings. Then we define a distance function(this can be considered the energy function), and we try to reduce the distance between the two views.

%Two views are usually two random augmentations of the same sample. In CV tasks, these augmentations are usually cropping out parts of the image, adding noise, scaling, rotation, flipping, color jitter, or a combination of a few augmentations. In order to increase the similarity of the two views, the networks should learn a transformation invariant embedding. In learning this transformation invariant embeddings, the network discovers important features or patterns that are useful in many downstream tasks.

%However, these kinds of Siamese networks suffer from a phenomenon called collapsing networks. If the network outputs the embedding for everything regardless of the input, energy between any two positive pairs will be reduced to zero. Researchers came up with different methods that use negative pairs to prevent collapsing. These methods are called Contrastive energy-based self-supervised learning. In addition to reducing the energy between positive pairs, they also try to increase the energy between two negative pairs. Usually, the two samples of the negative pair come from two different samples(regardless of their label). SimCLR is the most famous contrastive learning model that was introduced in recent history.

%Nevertheless, contrastive learning also has some issues, including training inefficiency. Non-Contrastive energy-based self-supervised models were introduced to overcome those issues. BYOL, SwAV, and SimSiam are some of the famous non-contrastive models that have been introduced recently.

%Aaqib et al. ~\cite{saeed2019multi} introduced self-supervised learning for time-series data by introducing augmentations that are compatible with time-series data. They use a Multi-Task Self-Supervised learning model to learn the embedding. They show their method's effectiveness using six human activity recognition data sets. Further details about this architecture will be discussed in the next section. Tang et al. ~\cite{tang2020exploring} have experimented with SimCLR architecture using HAR data. Qian et al. ~\cite{qian2022makes} explores BYOL, SimSiam, SimCLR, NNCLR, and TS-TCC on HAR data. The effectiveness of self-supervised learning on time-series data has already been proven over and over in recent years.

%The main reason for the introduction of self-supervised learning is the availability of vast unlabeled data and the difficulty of obtaining labeled data due to various reasons.

%User authentication using behavioral biometrics is one of the domains that suffers from the labeled data scarcity. Many privacy and security matters prevent researchers from obtaining and using labeled human biometric data. We can overcome most of these issues and build much better user authentication systems by utilizing the massive amounts of unlabelled data available. In this work, we focus on utilizing self-supervised learning to do so.

% \noindent{\bf 3. Efforts in behavioural biometrics to improve efficiency in use of training samples}\\ \vspace{-3mm} 

% \textcolor{red}{In the interest of space - we can move the relevant parts to above 2.1}

% Like most deep learning solutions, biometric user-authentication relies on a large amount of labelled training data. However collecting such large labelled datasets requires a significant amount of manual work which is often time-consuming and expensive. Within the user-authentication domain, labelled data also entails data privacy issues that can hinder the collection process. Furthermore, it is often not enough to simply collect data from many users but also ensure a sufficient number of samples is collected from each user. There are a few works which address this issue. 

 

% Solano et al.~\cite{solano2020few}, on the other takes a different approach by focusing on risk-based authentication scenario where the attacker holds a user’s authentication credentials and is trying to gain access to a system. The paper proposes a prototype using few-shot learning. This is motivated by the difficulty in gaining a sufficient number of training data for each user. The proposed approach is shown in the paper to give higher FRR and FAR measurements than the other methodologies it was compared to. However the authors demonstrated that the results were reasonable and still acceptable given that fewer training samples per user than the others. To exemplify, the proposed approach used at most seven logins per user while another method required 50. Nonetheless the difficulty of obtaining training data from multiple users was not a focus in this paper and  it is an aspect addressed in our work. 





% Although not directly focused on biometric user-authentication, the authors in ~\cite{saeed2019multi}  take a self-supervised approach for human activity detection. The paper implements an algorithm that jointly learns to solve multiple binary classification tasks where an original data sample is to be differentiated from one where a transformation has been applied to it.  In this way the deep neural network learns highly generalisable features from the available labelled data because in order to differentiate an original sample from a transformed one, it is made to learn the discriminatory characteristics of the original distribution of samples. We build upon this piece of work by experimenting the effectiveness of adding negative samples to each binary classification task. Our results reflect that our adaptation can improve the efficiency of the model in terms of the amount of labelled samples required for a downstream that can make use of the representation learned.



%The above examples require for the sensors to be embedded into smart devices. The collection of the user data and the pervasiveness of the application also depends largely on the device being used such as whether it is a smart watch or a desktop computer. There is however another collection of work on device-free user-authentication and depends on wireless sensing. These approaches, such as WiWho ~\cite{zeng2016wiwho} and BodyPIN ~\cite{wang2019continuous}, use commodity wifi for user identification or verification. While WiWho uses channel state information (CSI) to identify a person's walking gait, BodyPIN uses bio-electromagnetics to indicate a user's identity by sensing the impact of a human body by-passing WiFi signals. 
%\textcolor{red}{device-free authentication we can ignore.}


% The emergence of smart devices has ushered a wide range of research in the field of user authentication using biometric modalities. One type of biometric authentication requires sensors built into the devices which users interact with. Examples include TouchPass ~\cite{10.1145/3372224.3380901} which collects active vibration signal transmission through finger touch, MotionAuth ~\cite{yang2015motionauth} that uses motion sensors, BreathPrint ~\cite{chauhan2017breathprint} which uses microphone sensors to characterise an individual's breathing gestures and MusicID ~\cite{sooriyaarachchi2020musicid} which analyses music induced brain wave patterns for user identification and verification. 

% \textcolor{blue}{P1 - The pervasive use of smart devices and the vast amount sensitive information stored in those devices, exacerbate the problem of user authentication on smart devices. Traditional methods such as passwords, PINs, and security tokens have usability issues~\cite{} and static biometrics such as fingerprinting and face ID are vulnerable to spoofing attacks. As a result, \textit{behavioural biometrics} has been explored by many works as a more user friendly (i.e., implicit by nature and no extra effort is required from the user) and secure (i.e., difficult to spoof and allows continuous authentication) alternative for user authentication in smart devices.}

%Another key piece of work in the biometric authentication space combines deep learning models with online learning models ~\cite{chauhan2020contauth}. The motivation behind this work was to address a problem with generic biometric authentication methods, which is that the performance of these methods deteriorates when a user’s behaviour changes. Such temporal effects necessitates the re-training of the authentication model from scratch. However by combining deep learning models with online learning models, the authors use data incremental learning to address this problem and propose ContAuth. This new framework also implements class incremental learning to allow models to adapt when a new user needs to be authenticated. 


% \textcolor{red}{Self-supervised learning (SSL) is currently a highly active area of machine learning. 
% Self-supervised learning refers to the framework in which a model learns representations from unlabelled data with the use of a pretext task. Largely popular in the field of computer vision, the pretext task often involves training a model to learn to differentiate between an original unlabelled image sample and a transformed one (rotations, perturbations etc.) and the representations learned for this are then used in downstream tasks such as image classification.}


% P2 - The concept of self-supervised learning dates back to the mid-twentieth century. In 1978 Pal et al.~\cite{pal1978computer} used self-supervised to recognize vowel sounds. It is the oldest paper available on google scholar, which uses the term "self-supervised learning." Although the researchers did not directly use the term, many people experimented with this concept. In 1993 Bromley et al.~\cite{bromley1993signature} proposed the "Siamese" neural network architecture for signature verification. This "Siamese" network architecture paved the path to the success of most latest self-supervised architectures. Self-supervised learning overcomes the high labeled data requirement of deep learning models, making the bottleneck of computational resources. Due to the lack of computational resources, the concept of self-supervised learning died out in the twentieth century and resurfaced in the 2010s with the popularity of natural language processing. In 2013 Mikolov et al. ~\cite{mikolov2013distributed} used self-supervised learning to represent words in a vector space, famously known as word2vec. Inspired by word2vec, large-scale state-of-the-art NLP models such as BERT(Devlin et al.~\cite{devlin2018bert}), RoBERTa(Liu et al.~\cite{liu2019roberta}) and XLM-R(Conneau et al.~\cite{conneau2019unsupervised}) were developed. All these NLP models are masked language models, where we mask a part of a sentence or part of a paragraph and let the model predict the masked part. This masking method was not performing very well with computer vision tasks.

% With the resurrection of siamese networks in 2020 due to the popularity of SimCLR by Chen et al.~\cite{chen2020simple} self-supervised models for CV tasks started improving. Following the success of SimCLR,  SwAV(Caron et al.~\cite{caron2020unsupervised}), BYOL(Grill et al.~\cite{grill2020bootstrap}) and SimSiam(Chen et al.~\cite{chen2021exploring}) were proposed. Liu et al.~\cite{liu2021self} categorize all self-supervised methods into two categories, generative and contrastive. According to Yann LeCun's and Ishan Misra's blog post "Self-supervised learning: The dark matter of intelligence" on Meta AI Research, we cannot include SwAV, SimSiam, and BYOL in the contrastive category. They belong to the category of non-contrastive learning. It will be more accurate to categorize SSL methods into generative and comparative. Comparative methods can be again divided into contrastive and non-contrastive. All NLP models we mentioned belong to the generative category, and SimCLR belongs to the contrastive category.


%The general framework used in biometric-based authentication system ~\cite{abuhamad2020sensor} involves user enrollment where features acquired from data are used for modelling as well as the verification of the user which feeds extracted features to the authentication algorithm. Just as the type of signal/data collected has varied widely from breathing gestures to walking gaits, the algorithms used for authentication and identification has also varied between machine learning approaches such as SVM and decision trees, and deep learning approaches such as convolutional neural networks and long short-term memory networks~\cite{abuhamad2020sensor}.



% \textcolor{cyan}{Nonetheless, generative methods~\cite{hinton2006fast, kingma2013auto, goodfellow2014generative}(i.e. pretext task is to predict/generate a feature, a part of the input, or the whole input) were not successful with computer vision tasks because doing pixel-level generations are highly computationally expensive~\cite{chen2020simple}. Neither were discriminative approaches~\cite{doersch2015unsupervised, zhang2016colorful, noroozi2016unsupervised, gidaris2018unsupervised}(i.e. pretext task is to classify which transformation is applied to an input, given that finite number of transformations are applied to inputs) because they relies on heuristics to design pretext tasks limiting the generality of the learnt representation~\cite{chen2020simple}. Recent success in comparative models(i.e. pretext task try to increase the similarity/compatibility for given two positive pair) based on siamese networks~\cite{chen2020simple, grill2020bootstrap, caron2020unsupervised, chen2021exploring} has shown promising results in CV tasks.}

==> sections/SSL.tex <==
\section{Related Work - Extended}
In recent years self-Supervised gained a lot of popularity due to its' success in the domain of Natural Language processing. Some of the most famous language models that is trained using self-supervised learning are RoBERTa, XLM-R and BERT. In self-supervised learning we generate supervisory signal within our data by defining pre-text tasks. That is why the term "Unsupervised Learning" not in the use anymore.Because learning can never be unsupervised. In NLP models most commonly, the task is predicting a missing word in a middle of a sentence or predicting the next word of an unfinished sentence. There is a reason behind the success of NLP in self-supervised learning. There are only a finite number of words to select from to fill the blank. So these models can predict a probability distribution across all possible words and pick the word with the highest probability to complete the sentence. In other words, these pre-text tasks can be modeled as classification tasks. In contrast, computer vision tasks have an infinite number of possibilities. The task can be predicting a cropped-out part of an image, predicting a missing video frame, or predicting the next frame of a video. We have to do a pixel-level prediction of the missing part(part can be temporal or spatial).\\
In the past few years, self-supervised learning started improving its' performance in computer vision with the revival of Siamese Networks in 2019. These networks can be classified into the so-called Energy-Based Models(EBM) category. Yann LeCun and Ishan Misra talk about EBMs in their blog about self-supervised learning in their Meta AI blogpost. The term EBM is adapted from classical physics. In a high-level view, these models try to reduce the energy between two positive samples and increase the energy between two negative samples. This energy is usually a loss function or a distance function.\\
In Siamese networks, we have two identical networks. Sometimes one network can be a moving average of the other network. We try to reduce the energy between embeddings of two views of the same sample. We feed two views to the two identical networks. The outputs of the networks are the embeddings. Then we define a distance function(this can be considered the energy function), and we try to reduce the distance between the two views.\\
Two views are usually two random augmentations of the same sample. In CV tasks, these augmentations are usually cropping out parts of the image, adding noise, scaling, rotation, flipping, color jitter, or a combination of a few augmentations. In order to increase the similarity of the two views, the networks should learn a transformation invariant embedding. In learning this transformation invariant embeddings, the network discovers important features or patterns that are useful in many downstream tasks.\\
However, these kinds of Siamese networks suffer from a phenomenon called collapsing networks. If the network outputs the embedding for everything regardless of the input, energy between any two positive pairs will be reduced to zero. Researchers came up with different methods that use negative pairs to prevent collapsing. These methods are called Contrastive energy-based self-supervised learning. In addition to reducing the energy between positive pairs, they also try to increase the energy between two negative pairs. Usually, the two samples of the negative pair come from two different samples(regardless of their label). SimCLR is the most famous contrastive learning model that was introduced in recent history.\\
Nevertheless, contrastive learning also has some issues, including training inefficiency. Non-Contrastive energy-based self-supervised models were introduced to overcome those issues. BYOL, SwAV, and SimSiam are some of the famous non-contrastive models that have been introduced recently.\\
Aaqib et al. ~\cite{saeed2019multi} introduced self-supervised learning for time-series data by introducing augmentations that are compatible with time-series data. They use a Multi-Task Self-Supervised learning model to learn the embedding. They show their method's effectiveness using six human activity recognition data sets. Further details about this architecture will be discussed in the next section. Tang et al. ~\cite{tang2020exploring} have experimented with SimCLR architecture using HAR data. Qian et al. ~\cite{qian2022makes} explores BYOL, SimSiam, SimCLR, NNCLR, and TS-TCC on HAR data. The effectiveness of self-supervised learning on time-series data has already been proven over and over in recent years.\\
The main reason for the introduction of self-supervised learning is the availability of vast unlabeled data and the difficulty of obtaining labeled data due to various reasons.\\
User authentication using behavioral biometrics is one of the domains that suffers from the labeled data scarcity. Many privacy and security matters prevent researchers from obtaining and using labeled human biometric data. We can overcome most of these issues and build much better user authentication systems by utilizing the massive amounts of unlabelled data available. In this work, we focus on utilizing self-supervised learning to do so.\\
